Classical and quantum dynamical manifestations of index-2 saddles: concerted versus sequential reaction mechanisms

The presence of higher index saddles on a multidimensional potential energy surface is usually assumed to be of little significance in chemical reaction dynamics. Such a viewpoint requires careful reconsideration, thanks to elegant experiments and novel theoretical approaches that have come about in recent years. In this work, we perform a detailed classical and quantum dynamical study of a model two degree of freedom Hamiltonian, which captures the essence of the debate regarding the dominance of a concerted or a stepwise reaction mechanism. We show that the ultrafast shift of the mechanism from a concerted to a stepwise one is essentially a classical dynamical effect. In addition, due to the classical phase space being a mixture of regular and chaotic dynamics, it is possible to have a rich variety of dynamical behaviour, including a Murrell-Laidler type of mechanism, even at energies sufficiently above that of the index-2 saddle. We rationalize the dynamical results using an explicit construction of the classical invariant manifolds in the phase space.

==> engnames.tex <==
%
% engnames.tex 20.12.2006
%
\makeatletter
\def\contentsname{Contents}
\def\notesname{Notes}
\def\partname{Part}
\def\tocname{Contents}
\def\lofname{List of Figures}
\def\lotname{List of Tables}
\def\refname{REFERENCES}
\def\indexname{Index}
\def\figurename{Fig.}
\def\figuresname{Figures}%
\def\tablename{Table}
\def\tablesname{Tables}%
\def\abstractname{Abstract}
\def\appendixesname{Appendixes}%
\def\appendixname{Appendix}%
\def\acknowledgmentsname{Acknowledgments}
\def\journalname{??}
\def\copyrightname{??}
\def\andname{and}
\def\@pacs@name{MSC2010~numbers:}%
\def\@ydk@name{���~}%
\def\@keywords@name{Keywords:}%
\def\ppname{pp}
\def\numbername{number}
\def\volumename{volume}
\def\Dated@name{dated: }%
\def\Received@name{received }%
\def\Revised@name{in final form,~}%
\def\Accepted@name{accepted }%
\def\Published@name{published }%
\def\Presented@name{}%
%! 08.11.2006
\def\proofname{Proof}
\def\theoremname{Theorem}
\def\lemmaname{Lemma}
\def\propositionname{Proposition}
\def\assertionname{Assertion}
\def\corollaryname{Corollary}
\def\conjecturename{Conjecture}
\def\definitionname{Definition}
\def\remarkname{Remark}
\def\examplename{Example}
%!!
\makeatother
% ����� ����稪��
\makeatletter
\setcounter{teo}{0}
\setcounter{teon}{0}
\setcounter{lem}{0}
\setcounter{lemn}{0}
\setcounter{prp}{0}
\setcounter{prpn}{0}
\setcounter{ass}{0}
\setcounter{assn}{0}
\setcounter{cor}{0}
\setcounter{corn}{0}
\setcounter{hyp}{0}
\setcounter{hypn}{0}
\setcounter{proof}{0}
\setcounter{proofn}{0}
\setcounter{exa}{0}
\setcounter{exan}{0}
\setcounter{dfn}{0}
\setcounter{dfnn}{0}
\setcounter{rem}{0}
\setcounter{remn}{0}
\setcounter{problem}{0}
\setcounter{problemn}{0}
\setcounter{notat}{0}
\setcounter{notatn}{0}
\makeatother
\endinput


==> jpack_e.tex <==
%%
%% This is file  `jpack_e.tex',  Strelkov S.A.  20.12.2006
%%
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{amsfonts}
%\usepackage{oldlfont} %%% ���䫨����� � bm.sty
\usepackage{mathtext}
\usepackage[T2A,OT1]{fontenc}
\usepackage[cp1251,utf8]{inputenc}
\usepackage[russian,english]{babel}
%\usepackage{literat}
\usepackage{pifont}
\usepackage{bm}
\usepackage{array}
\usepackage{dcolumn}
\usepackage{hhline}
\usepackage{multirow}
\usepackage{graphicx}
\usepackage{epsfig,color}
\usepackage{rotating}
\usepackage{srcltx_p}
\usepackage{calc}
\usepackage{tabularx}
\usepackage{afterpage}
\usepackage{ifthen}
\usepackage{caption2n}
\usepackage{substr}
%\usepackage{minitoc} 
\usepackage{psfrag}
\usepackage[all]{xy}
\usepackage{mathrsfs}
%\usepackage{supertabular}
\RequirePackage{soul}
\RequirePackage[amsmath]{ntheorem}
\RequirePackage{verbatim}
%
\theoremseparator{.}
\theoremindent 0pt
\theorempreskipamount 6pt plus2pt minus2pt
\theorempostskipamount 6pt plus2pt minus2pt
%
\RequirePackage{enumerate}
\makeatletter
\setcaptionwidth{\linewidth}
\renewcommand{\captionlabeldelim}{.~}
\renewcommand{\captionlabelfont}{\bfseries}
\renewcommand{\captionfont}{\footnotesize}
\renewcommand \thefigure{\@arabic\c@figure}
\renewcommand \thetable{\@arabic\c@table}
\renewcommand{\arraystretch}{1.5}
\setlength{\extrarowheight}{2pt}
\setlength{\extratabsurround}{2pt}
%%% ��� � YADR.CLS
\renewcommand{\topfraction}{.90}
\renewcommand{\dbltopfraction}{.90}
\renewcommand{\bottomfraction}{.90}
\renewcommand{\textfraction}{0.10}
\renewcommand{\floatpagefraction}{0.90}
\renewcommand{\dblfloatpagefraction}{0.90}
\setcounter{topnumber}{4}
\setcounter{bottomnumber}{2}
\setcounter{totalnumber}{6}
%
\newcommand{\PreserveBackslash}[1]{\let\temp=\\#1\let\\=\temp}
\let\PBS=\PreserveBackslash
\def\settabpars#1#2#3{\vskip#1mm \tabcolsep=#2pt \def\arraystretch{#3}}
\newdimen\tabwidth\newdimen\tbwdth
\newcommand{\stretchtab}[2][1.0]{\setbox0=\hbox{\tabcolsep=0sp\ignorespaces#2}
          \setbox1=\hbox{\tabcolsep=1sp\ignorespaces#2}
          \tabwidth=#1\hsize \advance\tabwidth by -\wd0
          %\multiply\tabwidth by 1
          \tbwdth=\wd1\advance\tbwdth by -\wd0
          \divide\tabwidth by \tbwdth
          \tabcolsep=\tabwidth #2}
\newcommand\figcaption{\def\@captype{figure}\caption}
% 26.07.2006 \newcommand\tabcaption{\def\@captype{table}\caption}
\newcommand\tabcaption{\let\captionfont\small\def\@captype{table}\caption}
\renewcommand*\caption@@@normal{%
\parfillskip0pt plus 2fil%
  \caption@label\captiontext\par}
\newcaptionstyle{nonumber}{%
  \usecaptionmargin%
  \captionfont%
  \onelinecaption%
    {{\parbox[t]{\realcaptionwidth}{\parfillskip0pt plus 2fil\captiontext}}}%
    {\parfillskip0pt plus 2fil\captiontext}
}%
\newcommand{\commes}[1]{#1}
%\newcommand{\commes}[1]{\relax}
\def\place@bibnumber@inl#1{#1.}%
\flushbottom
\def\refitem#1{\relax}
%\def\refitem#1{\ifthenelse{\boolean{hmode}}{\protect\newline{}}{}\textbackslash{}refitem\{\hbox{\bfseries{}\itshape{}#1}\}\ifthenelse{\boolean{hmode}}{\protect\linebreak{}}{}}

\def\qedsymbol{\square}
\def\qed{\ifmmode\let\next\eqnqed\else
    \let\next\textqed\fi\next}
\def\eqnqed{\relax\eqno{\raisebox{-2mm}{\qedsymbol}}\ignorespaces}
\def\textqed{{\unskip\nobreak\hfil\penalty50\hskip1em\null\nobreak\hfil
    $\qedsymbol$\parfillskip\z@\finalhyphendemerits0\smallbreak\par}}
\def\p@subsubsection{}
\def\p@subsection{}
\def\p@section{}
\let\mtcSfont=\mtcSSfont
\def\l@section#1#2{%
 \addpenalty{1000}%
 \addvspace{0.4em plus 5\p@}%
 \@tempdima 2em %
 \begingroup\leftskip=-2em
  \parindent \z@ \rightskip \@tocrmarg
  \parfillskip -\rightskip
  \leavevmode %
  \advance\leftskip\@tempdima %
  \hskip -2em %
  #1\nobreak\hfil \nobreak\hb@xt@\@pnumwidth{\hss #2}\nopagebreak\par
 \endgroup
}%
\def\l@subsection#1#2{%
 \addpenalty{2000}%
 \addvspace{0em plus 1\p@}%
 \@tempdima=3em %
 \begingroup
  \leftskip=0em
  \parindent 0em \rightskip \@tocrmarg
  \parfillskip -\rightskip
  \leavevmode
  \advance\leftskip\@tempdima %
  \hskip -\leftskip %
  #1\nobreak\hfil \nobreak\hb@xt@\@pnumwidth{\hss #2}\nopagebreak\par
 \endgroup
}%
%\def\l@subsection{\@dottedtocline{2}{0em}{2.5em}}
\def\theequation{\arabic{section}.\arabic{equation}}
\@addtoreset{equation}{section}

\gdef\th@nonumberplain{%
  \def\@begintheorem##1##2{%
      \item[\hskip\labelsep \theorem@headerfont ##1.]}%
  \def\@opargbegintheorem##1##2##3{%
     \item[\hskip\labelsep \theorem@headerfont ##1\ {\upshape(}##3\/{\upshape)}.]}}

\renewcommand{\labelenumi}{$\theenumi.$}
\def\const{{\rm const}}

\makeatother
\endinput


==> maikdoi.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%             This is maikdoi.tex  V 1.2 22.10.2009
%
% ��࠭�祭��: ����� ࠡ����� ⮫쪮 � ISSN ������騬 �� ����;
%              ����� �������� \JournalISSNCode(1234-567X)
%              ��� \JournalCode(X2345671); ��� �஢�ન ����஫쭮� �㬬� ISSN.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\ProvidesFile{maikdoi.tex}
              [2009/10/23 v1.2
       add-on for MAIK document class revtex4n]
\typeout{revtex4n Class enhancement: maikdoi.tex for DOI}
%
\makeatletter
%
\def\JournalISSNnumber#1#2#3#4#5#6#7#8#9\@fin{\gdef\@JournalISSNnumber{#1#2#3#4#6#7#8#9}}
\expandafter\JournalISSNnumber\@JournalISSNCode\@fin
\typeout{JournalISSNnumber=\@JournalISSNnumber}
% macros to get and set the basic informations
%\def\journalnumber#1{\xdef\journ@lnumber{\padt@eight@digits{#1}}%
\def\journalnumber#1{\xdef\journ@lnumber{#1}%
%\checksize{journalnumber}8\journ@lnumber{99999999}%
}%
%\let\journ@lnumber=\empty
%
\def\ShortYear#1#2#3#4\@fin{\gdef\@ShortYear{#3#4}}
\expandafter\ShortYear\@TransYearOfIssue\@fin
\typeout{ShortYear=\@ShortYear}
\def\DOIyear#1{\xdef\DOI@year{\padt@two@digits{#1}}\checksize{DOIyear}2\DOI@year{99}}%
%
\def\DOIpsniy#1{\xdef\DOI@psniy{\padt@two@digits{#1}}% psniy - PublicationSerialNumberInYear
\checksize{DOIpsniy}2\DOI@psniy{99}}%
%
\def\DOIartnumber#1{\xdef\DOI@artnumber{\padt@three@digits{#1}}%
\checksize{DOIartnumber}3\DOI@artnumber{999}}
\def\DOI@artnumber{0}
%
\def\doitext#1{\xdef\doit@xtpref{#1}}
%
% a helpful hand of macros
\newif\if@wrongformat \@wrongformatfalse
%
\def\checksize#1#2#3#4{\ifnum#3>#4\PackageError{DOI2module}%
{Numeric value for "#1" to large!\MessageBreak
"#3" specified, but only #2 digits allowed}{Check your input!}
\@wrongformattrue \fi}
%
\newcount\modarg
\newcount\modmod
\newcount\tmp
\def\modulo{\tmp=\modarg\divide\modarg by\modmod\multiply\modarg
by\modmod\multiply\modarg by-1\global\advance\modarg by\tmp}
%
\def\padt@two@digits#1{\ifnum#1<10 0\fi\number#1}%
\def\padt@three@digits#1{\ifnum#1<100 0\fi%
\ifnum#1<10 0\fi\number#1}%
\def\padt@four@digits#1{\ifnum#1<1000 0\fi\ifnum#1<100 0\fi%
\ifnum#1<10 0\fi\number#1}%
\def\padt@five@digits#1{\ifnum#1<10000 0\fi\ifnum#1<1000 0\fi\ifnum#1<100 0\fi%
\ifnum#1<10 0\fi\number#1}%
\def\padt@eight@digits#1{\ifnum#1<1000000 0\fi\ifnum#1<1000000 0\fi\ifnum#1<100000 0%
\fi\ifnum#1<10000 0\fi\ifnum#1<1000 0\fi\ifnum#1<100 0\fi%
\ifnum#1<10 0\fi\number#1}%
%\def\setjahr#1{\xdef\jahr{#1}}
% @pii_digits_weights = (53,47,43,41,37,31,29,23,19,17,13,7,5,3,2);
\def\teilissn#1#2#3#4#5#6#7#8\@fin{%
\if#1X\modarg=10\relax\else\modarg=#1\relax\fi\multiply\modarg by53\advance\tmp by\modarg%
\if#2X\modarg=10\relax\else\modarg=#2\relax\fi\multiply\modarg by47\advance\tmp by\modarg%
\if#3X\modarg=10\relax\else\modarg=#3\relax\fi\multiply\modarg by43\advance\tmp by\modarg%
\if#4X\modarg=10\relax\else\modarg=#4\relax\fi\multiply\modarg by41\advance\tmp by\modarg%
\if#5X\modarg=10\relax\else\modarg=#5\relax\fi\multiply\modarg by37\advance\tmp by\modarg%
\if#6X\modarg=10\relax\else\modarg=#6\relax\fi\multiply\modarg by31\advance\tmp by\modarg%
\if#7X\modarg=10\relax\else\modarg=#7\relax\fi\multiply\modarg by29\advance\tmp by\modarg%
\if#8X\modarg=10\relax\else\modarg=#8\relax\fi\multiply\modarg by23\advance\tmp by\modarg}
\def\teilyear#1#2\@fin{%
\modarg=#1\relax\multiply\modarg by19\advance\tmp by\modarg%
\modarg=#2\relax\multiply\modarg by17\advance\tmp by\modarg}
\def\teilpsniy#1#2\@fin{%
\modarg=#1\relax\multiply\modarg by13\advance\tmp by\modarg%
\modarg=#2\relax\multiply\modarg by7\advance\tmp by\modarg}
\def\teilartnumber#1#2#3\@fin{%
\modarg=#1\relax\multiply\modarg by5\advance\tmp by\modarg%
\modarg=#2\relax\multiply\modarg by3\advance\tmp by\modarg%
\modarg=#3\relax\multiply\modarg by2\advance\tmp by\modarg}
%
% check for all required elements
\def\checkrequirements{
\if!\journ@lnumber!\typein[\answer]{^^JMissing 5-digit
journalnumber for the DOI, please specify:}\journalnumber\answer\fi
%
\ifnum\OF@year=0\typein[\answer]{^^JMissing 4-digit year for the OF
date, please specify:}\OFyear\answer\fi
%
\ifnum\DOI@year=0\typein[\answer]{^^JMissing 4-digit year for the DOI,
please specify:}\DOIyear\answer\fi
{\modarg=\DOI@year\relax\modmod=1000\relax\modulo
\expandafter\setjahr{\padt@three@digits\modarg}}
%
\if!\the\DOI@msnr!\typein[\answer]{^^JMissing 4-digit
manuscript number for the DOI, please specify:}\DOImsnr\answer\fi}
%
% make the package verbose
\def\showDOIargs{%
\typeout{^^JList of arguments for this DOI2 generation
^^J==========================================
^^JDOI-prefix :\space\maikpraefix
^^JISSN number:\space\journ@lnumber
^^JDOI-year\space\space\space:\space\DOI@year
^^JIn-Year-No.:\space\DOI@psniy
^^JArticle-No.:\space\DOI@artnumber
^^J==========================================}}
%
% perform the calculation
\def\DOIt{\if@wrongformat
   \typeout{Wrong format of at least one required value,^^Jno
            DOI could be generated.^^J}%
\else
   \edef\doit@xtcode{%
   \maikpraefix\journ@lnumber\DOI@year\DOI@psniy\DOI@artnumber}%
   \tmp=0\relax%
   \expandafter\teilissn\journ@lnumber\@fin%
   \expandafter\teilyear\DOI@year\@fin%
   \expandafter\teilpsniy\DOI@psniy\@fin%
   \expandafter\teilartnumber\DOI@artnumber\@fin%
   \modarg=\tmp\modmod=11\relax\modulo
   \ifnum\modarg<10\edef\checksum{\the\modarg}\else\edef\checksum{X}%
   \fi
   \edef\doit@xtcode{\doit@xtcode\checksum}
   \edef\doit@xt{\doit@xtpref\doit@xtcode}
   \showDOIargs
   \typeout{Calculated DOI:\space\space\doit@xtcode
   ^^J^^JVerbose:^^J\doit@xt^^J}
\fi
}
%
% set the defaults - the basics at least
%\def\springerpraefix{10.1007/s}
%!\def\maikpraefix{10.1134/S}
\doitext{\relax}%
%! 22.10.2009
\def\OnlineFirstDOI#1#2{\def\doit@xtcode{#1}%
\def\@onlinefirstdoi{#1}%
\def\@onlinefirstfilename{#2}%
\@booleantrue\onlinefirstdoi@sw%
\ifthenelse{\equal{\@nameincfi}{#2}}{%
\addtocounter{doiartnumber}{-\@ne}
}%
{\class@err{ ^^J^^J
\space\space \noexpand\OnlineFirstDOI{#1}{#2}^^J
\space\space Name Online First file:  #2^^J
\space\space Includepaper file name: \@nameincfi^^J
\space\space Not equal}%
}%
}%
%!!
%
\journalnumber{\@JournalISSNnumber}
\typeout{journalnumber=\journ@lnumber}
\DOIyear{\@ShortYear}
\typeout{DOIyear=\DOI@year}
\DOIpsniy{\@PublicationSerialNumberInYear}
\typeout{DOIpsniy=\DOI@psniy}
\makeatother
\endinput
%% End of file `maik.doi'


==> optn.tex <==
%%
%% This is file `optn.tex',  Strelkov S.A.  30.01.2002
%%
\begingroup
\catcode`\+\active\gdef+{\mathchar8235\nobreak\discretionary{}{\usefont{OT1}{cmr}{m}{n}\char43}{}}
\catcode`\-\active\gdef-{\mathchar8704\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char0}{}}
\catcode`\=\active\gdef={\mathchar12349\nobreak\discretionary{}{\usefont{OT1}{cmr}{m}{n}\char61}{}}
\endgroup
\def\cdot{\mathchar8705\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char1}{}}
\def\times{\mathchar8706\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char2}{}}
\mathcode`\==32768
\mathcode`\+=32768
\mathcode`\-=32768
% ����� ��⥬�����᪮�� ᨬ���� TeXBook ���� 185-186
% 2 --- �������� ��������
% 3 --- �⭮襭��
% <\equiv =\mathchar"3211>
\def \equiv   {\mathchar8721\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char17}{}}% "2211
% A.2.2~�������� �⭮襭��~LaTeX'a
% <\subseteq =\mathchar"3212>
\def \subseteq{\mathchar8722\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char18}{}} % "2222
% <\supseteq =\mathchar"3213>
\def \supseteq{\mathchar8723\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char19}{}}
\def \leq     {\mathchar8724\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char20}{}}
\def \geq     {\mathchar8725\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char21}{}}
\def \sim     {\mathchar8728\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char24}{}}
\def \approx  {\mathchar8729\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char25}{}}
\def \subset  {\mathchar8730\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char26}{}}
\def \supset  {\mathchar8731\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char27}{}}
\def \ll      {\mathchar8732\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char28}{}}
\def \gg      {\mathchar8733\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char29}{}}
\def \pm      {\mathchar8710\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char6}{}}
\def \mp      {\mathchar8711\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char7}{}}
\def \in      {\mathchar8754\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char50}{}}
\def \ni      {\mathchar8755\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char51}{}}
% ��. TeXBook ���. 510-511
% ��������� ᨬ���� ����� �����ୠ⨢��� �����, ������� ⠪ ��ப� �ᯮ��������,
% ��� plain TeX ����� ��� ��� �� ��� ��� ����� ��������� ��᫥����⥫쭮���:
% \ne ��� \neq (�� ��, ��� \not=)
% \le          (�� ��, ��� \leq)
% \ge          (�� ��, ��� \geq)
% (�� ��, ��� )
% (�� ��, ��� )
% (�� ��, ��� )
%<\prec =\mathchar"321E>
\def \prec    {\mathchar"321E\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"1E}{}}
%<\succ =\mathchar"321F>
\def \succ    {\mathchar"321F\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"1F}{}}
%<\preceq =\mathchar"3216>
\def \preceq  {\mathchar"3216\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"16}{}}
%<\succeq =\mathchar"3217>
\def \succeq  {\mathchar"3217\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"17}{}}
%<\simeq =\mathchar"3227>
\def \simeq  {\mathchar"3227\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"27}{}}
%<\cong =macro:->\mathrel {\mathpalette \@vereq \sim }>
%<\doteq =\long macro:->\DOTSB \mathrel {\mathop {\kern 0pt =}\limits ^{\textstyle .}}>
%<\sqsubseteq =\mathchar"3276>
\def \sqsubseteq {\mathchar"3276\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"76}{}}
%<\sqsupseteq =\mathchar"3277>
\def \sqsupseteq {\mathchar"3277\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"77}{}}
%<\smile =\mathchar"315E>
\def \smile   {\mathchar"315E\nobreak\discretionary{}{\usefont{OML}{cmm}{m}{n}\char"5E}{}}
%<\frown =\mathchar"315F>
\def \frown   {\mathchar"315F\nobreak\discretionary{}{\usefont{OML}{cmm}{m}{n}\char"5F}{}}
%<\perp =\mathchar"323F>
\def \perp    {\mathchar"323F\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"3F}{}}
%<\models =macro:->\mathrel {|}\joinrel \Relbar >
%<\mid =\mathchar"326A>
\def \mid     {\mathchar"326A\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"6A}{}}
%<\parallel =\mathchar"326B>
\def \parallel {\mathchar"326B\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"6B}{}}
%<\vdash =\mathchar"3260>
\def \vdash  {\mathchar"3260\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"60}{}}
%<\dashv =\mathchar"3261>
\def \dashv  {\mathchar"3261\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"61}{}}
%<\propto =\mathchar"322F>
\def \propto  {\mathchar"322F\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"2F}{}}
%<\asymp =\mathchar"3210>
\def \asymp  {\mathchar"3210\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"10}{}}
% latexsym
%<\sqsubset =\mathchar"3440>
\def \sqsubset {\mathchar"3440\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"40}{}}
%<\sqsupset =\mathchar"3441>
\def \sqsupset {\mathchar"3441\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"41}{}}
% A.2.2~�������� �⭮襭��~AMS
%<\leqslant =\mathchar"3436>
\def \leqslant {\mathchar"3436\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"36}{}}
%<\geqslant =\mathchar"343E>
\def \geqslant {\mathchar"343E\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"3E}{}}
%<\eqslantless =\mathchar"3430>
\def \eqslantless {\mathchar"3430\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"30}{}}
%<\eqslantgtr =\mathchar"3431>
\def \eqslantgtr {\mathchar"3431\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"31}{}}
%<\lesssim =\mathchar"342E>
%\def \lessim {\mathchar"342E\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"2E}{}}
%<\gtrsim =\mathchar"3426>
\def \gtrsim {\mathchar"3426\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"26}{}}
%<\lll =\mathchar"346E>
\def \lll {\mathchar"346E\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"6E}{}}
%<\ggg =\mathchar"346F>
\def \ggg {\mathchar"346F\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"6F}{}}
%<\lessgtr =\mathchar"3437>
\def \lessgtr {\mathchar"3437\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"37}{}}
%<\gtrless =\mathchar"343F>
\def \gtrless {\mathchar"343F\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"3F}{}}
%<\doteqdot =\mathchar"342B>
\def \doteqdot {\mathchar"342B\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"2B}{}}
%<\eqcirc =\mathchar"3450>
\def \eqcirc {\mathchar"3450\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"50}{}}
%<\circeq =\mathchar"3424>
\def \circeq {\mathchar"3424\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"24}{}}
%<\triangleq =\mathchar"342C>
\def \triangleq {\mathchar"342C\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"2C}{}}
%<\risingdotseq =\mathchar"343A>
\def \risingdotseq {\mathchar"343A\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"3A}{}}
%<\fallingdotseq =\mathchar"343B>
\def \fallingdotseq {\mathchar"343B\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"3B}{}}
%<\subseteqq =\mathchar"346A>
\def \subseteqq {\mathchar"346A\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"6A}{}}
%<\supseteqq =\mathchar"346B>
\def \supseteqq {\mathchar"346B\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"6B}{}}
%<\vartriangleleft =\mathchar"3443>
\def \vartriangleleft {\mathchar"3443\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"43}{}}
%<\vartriangleright =\mathchar"3442>
\def \vartriangleright {\mathchar"3442\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"42}{}}
% A.2.3~�������� �⭮襭��~AMS~�~����栭���
\def \neq      {\hbox{\text{\kern0.3em{\usefont{OMS}{cmsy}{m}{n}\char54}=}\kern0.3em}\nobreak\discretionary{}{{\usefont{OMS}{cmsy}{m}{n}\char54}=\kern0.3em}{}}
\let\ne=\neq
% <\nless =\mathchar"3504>
\def \nless   {\mathchar"3504\nobreak\discretionary{}{{\usefont{U}{msb}{m}{n}\char"04}}{}}
%<\in =\mathchar"3232>
%<\notin =macro:->\mathrel {\m@th \mathpalette \c@ncel \in }>
%<\nparallel =\mathchar"352C>
\def \nparallel {\mathchar"352C\nobreak\discretionary{}{\usefont{U}{msb}{m}{n}\char"2C}{}}
%<\nsubseteq =\mathchar"352A>
\def \nsubseteq {\mathchar"352A\nobreak\discretionary{}{\usefont{U}{msb}{m}{n}\char"2A}{}}
%<\nsupseteq =\mathchar"352B>
\def \nsupseteq {\mathchar"352B\nobreak\discretionary{}{\usefont{U}{msb}{m}{n}\char"2B}{}}
% A.3~��������~�����樨
%<\circ =\mathchar"220E>
\def \circ {\mathchar"220E\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"0E}{}}
%<\bigcirc =\mathchar"220D>
\def \bigcirc {\mathchar"220D\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"0D}{}}
%<\div =\mathchar"2204>
\def \div {\mathchar"2204\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"04}{}}
%<\diamond =\mathchar"2205>
\def \diamond {\mathchar"2205\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"05}{}}
%<\ast =\mathchar"2203>
\def \ast {\mathchar"2203\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"03}{}}
%<\star =\mathchar"213F>
\def \star {\mathchar"213F\nobreak\discretionary{}{\usefont{OML}{cmm}{m}{n}\char"3F}{}}
%<\cap =\mathchar"225C>
\def \cap {\mathchar"225C\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"5C}{}}
%<\cup =\mathchar"225B>
\def \cup {\mathchar"225B\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"5B}{}}
%<\sqcap =\mathchar"2275>
\def \sqcap {\mathchar"2275\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"75}{}}
%<\sqcup =\mathchar"2274>
\def \sqcup {\mathchar"2274\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"74}{}}
%<\wedge =\mathchar"225E>
\def \wedge {\mathchar"225E\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"5E}{}}
%<\vee =\mathchar"225F>
\def \vee {\mathchar"225F\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"5F}{}}
%<\oplus =\mathchar"2208>
\def \oplus {\mathchar"2208\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"08}{}}
%<\ominus =\mathchar"2209>
\def \ominus {\mathchar"2209\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"09}{}}
%<\otimes =\mathchar"220A>
\def \otimes {\mathchar"220A\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"0A}{}}
%<\odot =\mathchar"220C>
\def \odot {\mathchar"220C\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"0C}{}}
%<\Cap =\mathchar"2465>
\def \Cap {\mathchar"2465\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"65}{}}
%<\Cup =\mathchar"2464>
\def \Cup {\mathchar"2464\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"64}{}}
% A.4~��५��
%<\leftarrow =\mathchar"3220>
\def \leftarrow  {\mathchar"3220\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"20}{}}
%<\rightarrow =\mathchar"3221>
\def \rightarrow  {\mathchar"3221\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"21}{}}
%<\to =\mathchar"3221>
\def \to  {\mathchar"3221\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"21}{}}
%<\longleftarrow =\long macro:->\DOTSB \leftarrow \protect \joinrel \protect \relbar >
%<\longrightarrow =\long macro:->\DOTSB \protect \relbar \protect \joinrel \rightarrow >
%<\Leftarrow =\mathchar"3228>
\def \Leftarrow  {\mathchar"3228\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"28}{}}
%<\Rightarrow =\mathchar"3229>
\def \Rightarrow  {\mathchar"3229\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"29}{}}
%<\Longleftarrow =\long macro:->\DOTSB \Leftarrow \protect \joinrel \protect \Relbar >
%<\Longrightarrow =\long macro:->\DOTSB \protect \Relbar \protect \joinrel \Rightarrow >
%<\leftrightarrow =\mathchar"3224>
\def \leftrightarrow  {\mathchar"3224\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"24}{}}
%<\longleftrightarrow =\long macro:->\DOTSB \leftarrow \joinrel \rightarrow >
%<\Leftrightarrow =\mathchar"322C>
\def \Leftrightarrow  {\mathchar"322C\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"2C}{}}
%<\Longleftrightarrow =\long macro:->\DOTSB \Leftarrow \joinrel \Rightarrow >
%<\uparrow =macro:->\delimiter "3222378 >
%<\downarrow =macro:->\delimiter "3223379 >
%<\Uparrow =macro:->\delimiter "322A37E >
%<\Downarrow =macro:->\delimiter "322B37F >
%<\updownarrow =macro:->\delimiter "326C33F >
%<\Updownarrow =macro:->\delimiter "326D377 >
%<\leftleftarrows =\mathchar"3412>
\def \leftleftarrows {\mathchar"3412\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"12}{}}
%<\rightrightarrows =\mathchar"3413>
\def \rightrightarrows {\mathchar"3413\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"13}{}}
%<\leftrightarrows =\mathchar"341C>
\def \leftrightarrows {\mathchar"341C\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"1C}{}}
%<\rightleftarrows =\mathchar"341D>
\def \rightleftarrows {\mathchar"341D\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"1D}{}}
%<\upuparrows =\mathchar"3414>
\def \upuparrows {\mathchar"3414\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"14}{}}
%<\downdownarrows =\mathchar"3415>
\def \downdownarrows {\mathchar"3415\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"15}{}}
%<\nLeftarrow =\mathchar"353A>
\def \nLeftarrow {\mathchar"353A\nobreak\discretionary{}{\usefont{U}{msb}{m}{n}\char"3A}{}}
%<\nRightarrow =\mathchar"353B>
\def \nRightarrow {\mathchar"353B\nobreak\discretionary{}{\usefont{U}{msb}{m}{n}\char"3B}{}}
\endinput
%\DeclareFontEncoding{OML}{}{}
%\DeclareFontEncoding{OMS}{}{}
%\DeclareFontEncoding{OMX}{}{}
%\DeclareFontEncoding{U}{}{\noaccents@}
%\DeclareFontSubstitution{OML}{cmm}{m}{it}
%\DeclareFontSubstitution{OMS}{cmsy}{m}{n}
%\DeclareFontSubstitution{OMX}{cmex}{m}{n}
%\DeclareFontSubstitution{U}{cmr}{m}{n}

